Deep Set Prediction Networks

Current approaches for predicting sets from feature vectors ignore the unordered nature of sets and suffer from discontinuity issues as a result. We propose a general model for predicting sets that properly respects the structure of sets and avoids this problem. With a single feature vector as input, we show that our model is able to auto-encode point sets, predict the set of bounding boxes of objects in an image, and predict the set of attributes of these objects.

==> table-0.tex <==

\begin{tabular}{ccccc}
\toprule
$\hat{\bm{Y}}^{(5)}$ & $\hat{\bm{Y}}^{(10)}$ & $\hat{\bm{Y}}^{(20)}$ & True $\bm{Y}$ & Baseline\\
\midrule
(-0.80, -0.12, 3.11) & (-2.41, -1.77, 0.27) & (-2.66, 1.82, 0.45) & (-2.82, 1.95, 0.35) & (-2.56, 2.16, 0.35)\\
small gray metal \textcolor{red}{sphere} & small \textcolor{red}{red} metal \textcolor{red}{sphere} & small gray metal cube & small gray metal cube & small \textcolor{red}{red} metal \textcolor{red}{cylinder}\\
(-0.18, -0.33, 3.34) & (-1.98, 1.74, 0.39) & (-2.26, -2.05, 0.29) & (-2.37, -2.18, 0.35) & (-2.52, -2.53, 0.37)\\
\textcolor{red}{large} \textcolor{red}{gray} metal sphere & small \textcolor{red}{gray} metal \textcolor{red}{cube} & small red metal sphere & small red metal sphere & small \textcolor{red}{gray} metal sphere\\
(0.06, 0.85, 3.54) & (-1.60, -0.20, 0.61) & (-1.44, 0.10, 0.61) & (-1.55, 0.22, 0.70) & (-1.58, 1.40, 0.71)\\
large \textcolor{red}{gray} metal sphere & large red metal sphere & large red metal sphere & large red metal sphere & large \textcolor{red}{yellow} metal sphere\\
(0.14, -0.07, 3.36) & (-1.02, 2.44, 0.54) & (-1.03, 2.26, 0.63) & (-1.33, 2.34, 0.70) & (-0.86, 0.28, 0.69)\\
large gray \textcolor{red}{rubber} \textcolor{red}{sphere} & large gray metal cylinder & large gray metal cylinder & large gray metal cylinder & large \textcolor{red}{purple} metal \textcolor{red}{sphere}\\
(0.60, 1.41, 3.45) & (-0.82, -1.96, 0.61) & (-0.69, -2.07, 0.70) & (-0.69, -2.27, 0.70) & (-0.28, -1.84, 0.70)\\
large gray \textcolor{red}{metal} \textcolor{red}{cylinder} & large gray rubber sphere & large gray rubber sphere & large gray rubber sphere & large \textcolor{red}{yellow} rubber sphere\\
(1.03, -0.95, 3.08) & (0.80, -2.50, 0.29) & (0.86, -2.62, 0.30) & (0.95, -2.83, 0.35) & (1.31, -2.55, 0.35)\\
small \textcolor{red}{purple} rubber cube & small yellow rubber cube & small yellow rubber cube & small yellow rubber cube & small \textcolor{red}{gray} rubber cube\\
\bottomrule
\end{tabular}

